DG-SLAM: Robust Dynamic Gaussian Splatting SLAM with Hybrid Pose Optimization

Achieving robust and precise pose estimation in dynamic scenes is a significant research challenge in Visual Simultaneous Localization and Mapping (SLAM). Recent advancements integrating Gaussian Splatting into SLAM systems have proven effective in creating high-quality renderings using explicit 3D Gaussian models, significantly improving environmental reconstruction fidelity. However, these approaches depend on a static environment assumption and face challenges in dynamic environments due to inconsistent observations of geometry and photometry. To address this problem, we propose DG-SLAM, the first robust dynamic visual SLAM system grounded in 3D Gaussians, which provides precise camera pose estimation alongside high-fidelity reconstructions. Specifically, we propose effective strategies, including motion mask generation, adaptive Gaussian point management, and a hybrid camera tracking algorithm to improve the accuracy and robustness of pose estimation. Extensive experiments demonstrate that DG-SLAM delivers state-of-the-art performance in camera pose estimation, map reconstruction, and novel-view synthesis in dynamic scenes, outperforming existing methods meanwhile preserving real-time rendering ability.

==> fig/vis_compare.tex <==
\begin{figure}[t]
% \vspace{-8mm}
\begin{center}
\includegraphics[width=0.99\textwidth, height=0.77\textwidth]{fig/vis_compare/vis_mesh_V4.pdf}
\put(-298,5){{\texttt{move\_no\_box2}} }
\put(-188,5){\texttt{walk\_xyz}}
\put(-93,5){\texttt{person\_track2} }
\put(-338,218){\rotatebox{90}{ESLAM}}
\put(-338,151){\rotatebox{90}{Co-SLAM}}
\put(-338,99){\rotatebox{90}{Ours}}
\put(-338,34){\rotatebox{90}{TSDF}}
\end{center}
% \vspace{-4mm}
 \caption{\textbf{Visual comparison of the reconstructed meshes on the \textit{BONN} and \textit{TUM RGB-D} datasets.} Our results are more complete and accurate without the dynamic object floaters. More examples are in the appendix.}
\label{fig:vis_compare}
% \vspace{-2mm}
\end{figure}

==> table/ablation.tex <==
\begin{table}[h]
\begin{minipage}{\textwidth}

\begin{minipage}[t]{0.45\textwidth}
\makeatletter\def\@captype{table}
\renewcommand\tabcolsep{1.8pt}
\renewcommand\arraystretch{1.0}
\footnotesize
%\resizebox{.95\linewidth}{!}{
\begin{center}
\centering
\begin{tabular}{l cc}
\toprule[2pt] 
  & ATE[cm]$\downarrow$ & STD[cm]$\downarrow$\\
\midrule
\midrule

w/o Add & 6.63 &3.08\\
w/o Prune & 6.89 &3.16\\
w/o Dep. Warp &6.40 &3.22\\
w/o Seg &15.27 &7.47\\
w/o Fine Tracking &7.36 &3.62\\
DG-SLAM(Ours) & \textbf{5.51} & \textbf{2.79}\\
\bottomrule[2pt]
\end{tabular}
\vspace{1mm}
\caption{\textbf{Ablation study on \textit{BONN} dataset.}}
\label{ablation_study}
\end{center}
\end{minipage}
\begin{minipage}[t]{0.58\textwidth}
\makeatletter\def\@captype{table}
\renewcommand\tabcolsep{1.8pt}
\renewcommand\arraystretch{1.0}
\footnotesize
\centering
\begin{tabular}{l ccc}
\toprule[2pt] 
 & Tracking & Mapping & Avg. Running\\
  % & Track.[ms]$\downarrow$ & Map.[ms]$\downarrow$ & Avg. Run.[ms] $\downarrow$ \\
    & [ms]$\downarrow$ &[ms]$\downarrow$ & [ms] $\downarrow$ \\
\midrule
\midrule
NICE-SLAM \cite{nice_slam}& 3186.2 &1705.1 &4892.3\\
ESLAM \cite{eslam}&2045.9 &1641.4 &3688.5\\
Point-SLAM \cite{Sandström2023ICCV} &2279.5  &1544.4&3823.9\\
Co-SLAM \cite{co-slam}&101.4 &\textbf{140.1} &\textbf{241.6}\\
DG-SLAM(Ours) & \textbf{89.2}  & 549.3& 645.9 \\
\bottomrule[2pt]
\end{tabular}
\vspace{1mm}
\caption{\textbf{Run-time comparison
on \textit{TUM} f3/w\_s.}}
\label{Run_time}
\end{minipage}
\end{minipage}
% \vspace{-2mm}
\end{table}

==> table/scannet.tex <==
\begin{table}[h]
\begin{minipage}{\textwidth}

\begin{minipage}[t]{0.58\textwidth}
\makeatletter\def\@captype{table}
\renewcommand\tabcolsep{1.5pt}
\renewcommand\arraystretch{1.0}
\small
%\resizebox{.95\linewidth}{!}{
\begin{center}
\centering
\begin{tabular}{l cccccc   c}
\toprule[2pt] 
Method & 00 & 59 & 106 & 169 & 181 & 207 & Avg.\\
\midrule
\midrule
NICE-SLAM \cite{nice_slam}& 12.0 &14.0& 7.9& 10.9& 13.4& 6.2& 10.7 \\
Co-SLAM \cite{co-slam}& \textbf{7.1} &11.1& 9.4& \textbf{5.9}& 11.8& \textbf{7.1}& 8.8\\
Point-SLAM \cite{Sandström2023ICCV} &10.2 &7.8&8.7& 22.2& 14.8& 9.5& 12.2\\
% \midrule
SplaTAM \cite{keetha2023splatam} &12.8 &10.1&17.7& 12.1& 11.1& 7.5& 11.9\\
GS-SLAM \cite{matsuki2023gaussian} &13.6 &\textbf{7.6}&8.1& 13.7& 34.6& 12.5&15.1 \\
% \rowcolor{lime!20}
DG-SLAM(Ours) & 7.9 & 11.5 & \textbf{8.0} & 8.3 & \textbf{7.3} & 8.2 & \textbf{8.6} \\
\bottomrule[2pt]
\end{tabular}
\vspace{1mm}
\caption{\textbf{Camera tracking results on \textit{ScanNet}.} The \\ metric is  ATE and the unit is [cm].}
\label{scannet}
\end{center}
\end{minipage}
\begin{minipage}[t]{0.38\textwidth}
\makeatletter\def\@captype{table}
\renewcommand\tabcolsep{1.5pt}
\renewcommand\arraystretch{1.0}
\small
% \begin{center}
%\resizebox{.95\linewidth}{!}{
\centering
\begin{tabular}{l cc}
\toprule[2pt] 
Iterations & tracking & mapping\\
\midrule
\midrule

NICE-SLAM \cite{nice_slam}& 200 &60\\
Co-SLAM \cite{co-slam}& \textbf{20} &\textbf{30}\\
ESLAM \cite{eslam}&200 &60\\
Point-SLAM \cite{Sandström2023ICCV} &200 &150\\
SplaTAM \cite{keetha2023splatam} &200 &\textbf{30}\\

GS-SLAM \cite{matsuki2023gaussian} &100 &81\\
DG-SLAM(Ours) & \textbf{20} & 40\\
\bottomrule[2pt]
\end{tabular}
\vspace{1mm}
\caption{\textbf{Running iterations on \textit{TUM}.}}
\label{iterations}
\end{minipage}
\end{minipage}
\vspace{-2mm}
\end{table}
